Stage-based Hyper-parameter Optimization for Deep Learning

As deep learning techniques advance more than ever, hyper-parameter optimization is the new major workload in deep learning clusters. Although hyper-parameter optimization is crucial in training deep learning models for high model performance, effectively executing such a computation-heavy workload still remains a challenge. We observe that numerous trials issued from existing hyper-parameter optimization algorithms share common hyper-parameter sequence prefixes, which implies that there are redundant computations from training the same hyper-parameter sequence multiple times. We propose a stage-based execution strategy for efficient execution of hyper-parameter optimization algorithms. Our strategy removes redundancy in the training process by splitting the hyper-parameter sequences of trials into homogeneous stages, and generating a tree of stages by merging the common prefixes. Our preliminary experiment results show that applying stage-based execution to hyper-parameter optimization algorithms outperforms the original trial-based method, saving required GPU-hours and end-to-end training time by up to 6.60 times and 4.13 times, respectively.

==> Makefile <==
TEXFILE=hippo.tex
TARGET=hippo
TEXFILES=$(wildcard *.tex)
BIBFILES=hippo.bib
FIGFILES=$(wildcard figures/*.pdf) $(wildcard figures/*.eps)

all: ${TARGET}.pdf

${TARGET}.pdf: ${TEXFILES} ${BIBFILES} ${FIGFILES} ${TARGET}.bbl
	( \
	pdflatex $(TARGET).tex; \
	while grep -q "Rerun to get cross-references right." $(TARGET).log; \
	do \
		pdflatex $(TARGET).tex; \
	done \
	)

${TARGET}.bbl: ${TARGET}.bib
	pdflatex ${TARGET}.tex
	bibtex ${TARGET}
	pdflatex ${TARGET}.tex
	pdflatex ${TARGET}.tex

.PHONY: clean
clean:
	rm -f \
	$(TEXFILE:.tex=.aux) \
	$(TEXFILE:.tex=.log) \
	$(TEXFILE:.tex=.out) \
	$(TEXFILE:.tex=.dvi) \
	$(TEXFILE:.tex=.pdf) \
	$(TEXFILE:.tex=.thm) \
	$(TEXFILE:.tex=.bbl) \
	$(TEXFILE:.tex=.blg) \
	$(TEXFILE:.tex=.ps) \
	$(TEXFILE:.tex=.ent) \
	latex.out/* \
	figures/*-eps-converted-to.pdf

.PHONY: build
build:
	@bin/latexrun $(TARGET)

